MIST: Defending Against Membership Inference Attacks Through Membership-Invariant Subspace Training

In Member Inference (MI) attacks, the adversary try to determine whether an instance is used to train a machine learning (ML) model. MI attacks are a major privacy concern when using private data to train ML models. Most MI attacks in the literature take advantage of the fact that ML models are trained to fit the training data well, and thus have very low loss on training instances. Most defenses against MI attacks therefore try to make the model fit the training data less well. Doing so, however, generally results in lower accuracy. We observe that training instances have different degrees of vulnerability to MI attacks. Most instances will have low loss even when not included in training. For these instances, the model can fit them well without concerns of MI attacks. An effective defense only needs to (possibly implicitly) identify instances that are vulnerable to MI attacks and avoids overfitting them. A major challenge is how to achieve such an effect in an efficient training process. Leveraging two distinct recent advancements in representation learning: counterfactually-invariant representations and subspace learning methods, we introduce a novel Membership-Invariant Subspace Training (MIST) method to defend against MI attacks. MIST avoids overfitting the vulnerable instances without significant impact on other instances. We have conducted extensive experimental studies, comparing MIST with various other state-of-the-art (SOTA) MI defenses against several SOTA MI attacks. We find that MIST outperforms other defenses while resulting in minimal reduction in testing accuracy.

==> backup_files/intro_first_version.tex <==

\section{Introduction}
Machine learning models are now prevalent in our daily lives, from voice assistants~\cite{lopez2018alexa}, to image generation~\cite{ramesh2021zero}, to chatbots (e.g., ChatGPT-4~\cite{openai2023gpt4}). These large neural networks are powerful but also susceptible to security and privacy issues, such as whether personal data used to train these models is not being leaked by these large models. There are mainly two types of privacy-threatening inference attacks against individual training samples: The first one is the membership inference (MI) attack~\cite{shokri2017membership,nasr2019comprehensive}, where an adversary seeks to infer if a given instance was part of the training data; the second one is the instance reconstruction attack~\cite{salem2020updates,fredrikson2015model}, where the adversary seeks to reconstruct each sample as perfectly as possible. Our work focuses on membership inference attacks. Essentially, if the optimal membership inference attack is merely as good as random guessing, then there is no privacy leakage in the sense of differential privacy~\cite{li2013membership}.

\paragraph{Threat model} Our work  focuses on blackbox membership inference attacks of classifiers, where the adversary can only feed a query into the target model and get a (softmax) prediction. This is the hardest setting for the adversary and the most common setting is real world applications where users have access to an API (e.g., OpenAI's GPT-4 API~\cite{openai2023gpt4}). 
%
Existing blackbox membership inference attacks can be categorized into three classes: loss based MI attacks~\cite{shokri2017membership,yeom2018privacy,carlini2021membership,song2019membership,long2017towards,watson2021importance,ye2021enhanced}, perturbation based attacks~\cite{jayaraman2020revisiting} and set based attacks~\cite{hui2021practical}. 

\paragraph{A short summary of existing works}
The basic intuition of loss-based blackbox MI attacks is that large machine learning models tend to overfit the training data, thus having smaller loss on training instances than testing instances. 
%Based on this idea, Yeom et al.~\cite{yeom2018privacy} proposed the blackbox loss attack, where one instance is predicted to be a member when its loss is lower than a fixed threshold. Shokri et al.~\cite{shokri2017membership} suggested to train an attack model per class to achieve higher accuracy and the input to the attack model should be the whole prediction instead of just one loss. Furthermore, researchers noticed that the hardness of membership inference on different instances is different, which implies that training one attack model for each particular instance can improve attack effectiveness. 
Moreover, Watson et al.~\cite{watson2021importance} shows that each training instance has a different MI hardness. More specifically, there are some training instances that have low loss when used in training and have high loss when not used in training, thus being easier to be detected by MI attacks. 
%Ye et al.~\cite{ye2021enhanced} pointed out that the attack from ~\cite{watson2021importance} cannot choose a FPR (false positive rate) as they wish to launch the attack. To tackle this issue, Ye et al.~\cite{ye2021enhanced} proposed to train multiple shadow models with or without a particular instance, thus getting a member loss set and a nonmember loss set. By leveraging a one-side hypothesis testing, the attacker is able to choose an appropriate FPR to launch the attack. However, the attacker needs to train a huge amount of shadow models if the desired FPR is extremely low, for example $0.01\%$.  
Carlini et al.~\cite{carlini2021membership} argued that the average-case metrics such as accuracy and AUC score fail to characterize whether the attack can confidently identify any members of the training set. To confidently identify members, true positive rate at a fixed low false positive rate (e.g. $0.1\%$) should be used to evaluate the effectiveness of different attacks. To make MI attacks effective at extremely low FPR region, Carlini et al.~\cite{carlini2021membership} proposed LIRA, a likelihood ratio attack, which obtains the distribution of outputs of  member and nonmember losses (which are shown to be approximately normal distributions). In LIRA the attacker uses a likelihood ratio test to estimate whether the output of the model for a specific instance is drawn from the member distribution or the nonmember distribution. We include a detailed explanation of these and other types of MI attacks in \Cref{sec:mi_attacks_summary}.
The CANARY attack~\cite{wen2022canary} proposed one updated version of LIRA: CANARY suggests that, by querying the given target instance with adversarially crafted noise, it achieves higher true positive rate at a fixed low false positive rate and higher attack AUC.
%Since there is a single metric for all instances, the attacker only needs to train enough shadow models to estimate the prediction distributions accurately, which requires much less computational resources than ~\cite{ye2021enhanced}. 

%The intuition of the noise based attacks is that, training data needs more random perturbations to flip its label than testing data, since the target model is well trained with augmented training data. The attack from ~\cite{jayaraman2020revisiting} proposed to add many different random gaussian noise to a given instance and count the number of times that the predicted label is flipped. If the count is less a given threshold, then this instance is predicted as a member.

%The intuition of the set based attacks is that the predictions of member instances are more close to each other, leading to lower MMD (mean maximum discrepancy) distance in this set. If the attacker add one nonmember prediction to the member set, then the MMD distance would increase. They proposed an iterative method to generate member set and nonmember set and finally the instances in the member set is the predicted members.

As for defenses, in Shokri et al.~\cite{shokri2017membership} proposed the use of $L_2$-regularization on the model parameters to reduce ovefitting and defend against blackbox MI attacks, which works for small models but it is generally not as effective in large neural network models. Nasr et al.~\cite{nasr2018machine} proposes an adversarial regularization, which trains an attacker model on the fly and tries to minimize the attack accuracy so that the privacy leakage of the target model is minimized. Jia et al.~\cite{jia2019memguard} proposes to train an attacker model after the training of the target model and add intentionally crafted noise to each prediction to fool the trained attack model. However, both Nasr's defense and Jia's defense can only defend a particular attacker during the training, leaving the target model unprotected against other attackers. 
Li et al.~\cite{li2020membership} uses a distribution loss (maximum mean discrepancy (MMD)) to regularize the model and minimize the difference between the distribution of member and nonmember predictions. Li et al.\ also suggests to use mix-up data augmentation to simultaneously reduce the training accuracy and increase the testing accuracy (reducing the overfitting). Tang et al.~\cite{tang2022mitigating} proposes a novel ensemble architecture called SELENA, which trains a set of models and only use models that are not trained with a particular instance to give the prediction of that instance. In essence, the goal of these existing defenses are two-fold: better generalization ($L_2$ regularization, mix-up data augmentation) and reducing the gap between the distribution of member and nonmember predictions from the model. However, CANARY attack~\cite{wen2022canary} shows that there is no effective defenses against blackbox MI attacks at low FPR regions. In this paper we introduce, to the best of our knowledge, an effective defense against blackbox MI attacks at low FPR regions.

To defend against blackbox MI attacks that target the most vulnerable instances such as LIRA and CANARY, we need to focus on the vulnerability of every particular instance in the training data (rather than just general model prediction distributions as prior work). From a differential privacy perspective, we would like to have one classifier that can give the same prediction for any given data instance no matter if we include this data instance in the training or not and no matter what the rest of of the training set looks like. However, the most recent theoretical results (e.g., Abadi et al.~\cite{abadi2016deep}) show that such a differentially-private model would suffer a huge testing accuracy drop.
Hence, we explore a more empirically-focused defense against blackbox MI attacks on the most vulnerable instances that relaxes the strict differentially privacy guarantees.

\paragraph{Proposed solution}
We start by relaxing the restrictions imposed by differential privacy. given a training set $D$, for any single data instance $(x_M,y_M) \in D$, we would like to have a classifier that gives the same prediction for any data instance from a given support $\Omega$ when trained using $D$ and when trained using $D \setminus \{(x_M,y_M)\}$. Here $(x_M,y_M)$ can be any data instance from the training set $D$ and we would like to have the classifier to satisfy this restriction for all data instances in $D$. 
This classifier invariance to changing $D$ by one instance is a special (simple) case type of counterfactually-invariant representation learning~\cite{mouli2022asymmetry,quinzan2022learning,veitch2021counterfactual,jiang2022invariant}, which we will expand on this in \Cref{sec:proposal}.
Unfortunately, learning this invariance with standard methods is still challenging, since each training instance induces a set of restrictions in learning the classifier, this would require a complex loss function over $n$ leave-one-out datasets from $D$, which is computationally infeasible for anything but a very small neural network model. 

To tackle this challenge, we propose \EiSL (Membership-Invariant Subspace Training).
\EiSL uses a novel two-phase subspace learning procedure that trains models regularized to be counterfactually invariant to the membership of each instance in the training data $D$.
We denote this invariant classifier training procedure {\em membership-invariance} learning.
The algorithm behind \EiSL is detailed in \Cref{sec:proposal}.

% the cross-difference loss, which is to measure the maximum prediction difference for a model $F$ on any given data instance $(x,y)$ from  a given support $\Omega$ when trained using $D$ and when trained using $D \setminus \{(x_M,y_M)\}$. We consider the cross-difference loss for all $(x_M,y_M) \in D$. In other words, if this cross-difference loss of one model $F$ is $0$ for all $(x_M,y_M) \in D$, then this model $F$ is environment-invariant on $D$, which is the ideal model we would like to have. Next, we realize that the subspace learning can be utilized to facilitate the computation of the cross-difference loss in an approximated way. The core idea of subspace learning is that subspace learning optimizes models in a parameter subspace that contains diverse solutions that can be integrated and ensembled to achieve higher accuracy, better calibration and more robustness to noise. Suppose there are $K$ submodels, then each submodel in this subspace is trained using a disjoint subset $D_k$ from the original training set $D$. With these diverse models from subspace learning, the cross-difference loss can be approximated calculated. Therefore, these diverse models can be regularized by the cross-difference loss, which implies that these diverse models are becoming more environment-invariant, thus more robust against MI attacks. Besides, subspace learning methods have been proven to provide better generalization, which can also help defend against MI attacks.

%Furthermore, we suggest the model trainers to use Mix-up data augmentation to further defend against MI attacks when applicable.

%In the most ideal case, the LIRA attack can be reduced to the loss attack proposed in ~\cite{yeom2018privacy}.

\mypara{Contributions.} 

\begin{enumerate}[leftmargin=*] 
\item We propose the \textbf{Membership-Invariant Subspace Training} (\EiSL) defense designed to specifically defend against blackbox membership inference attacks on the most vulnerable instances in the training data (which also helps defending against overall blackbox MI attacks). \EiSL uses a novel two-phase subspace learning procedure that trains models regularized to be counterfactually invariant to the membership of each instance in the training data $D$.
\item We compare our defenses against baselines and provide extensive experiments showing that our defense can significantly reduce the effectiveness of existing membership inference attacks.
To the best of our knowledge, \EiSL is the first effective defense against LIRA and CANARY-style blackbox MI attacks that focuses on defending the most vulnerable instances in the training data, while improving the overall MI attack robustness.
\end{enumerate}


\mypara{Roadmap.} The rest of this paper is organized as follows. In section \ref{sec:prelim}, we introduce some machine learning background and summarize existing membership inference attacks and defenses in centralized setting. In section \ref{sec:defense}, we propose our new defense, the \textbf{Membership-Invariant Subspace Training} (\EiSL) defense. In section \ref{sec:experiments}, we present our extensive experimental evaluations and compare our proposed defense with existing defenses. 
%In section \ref{sec:related}, we list and summarize further related works. 
In section \ref{sec:conclusion}, we conclude this paper.
